Deriving Law-Abiding Instances

Liquid Haskell's refinement-reflection feature augments the Haskell language with theorem proving capabilities, allowing programmers to retrofit their existing code with proofs. But many of these proofs require routine, boilerplate code that is tedious to write. Moreover, many such proofs do not scale well, as the size of proof terms can grow superlinearly with the size of the datatypes involved in the proofs. We present a technique for programming with refinement reflection which solves this problem by leveraging datatype-generic programming. Our observation is that we can take any algebraic datatype, generate an equivalent representation type, and have Liquid Haskell automatically construct (and prove) an isomorphism between the original type and the representation type. This reduces many proofs down to easy theorems over simple algebraic "building block" types, allowing programmers to write generic proofs cheaply and cheerfully.

==> haskell_style.tex <==
\usepackage{upquote}
\usepackage{listings}
% This is used in the acmart.cls, leading to problems with option clash:
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage[dvipsnames]{xcolor}
\usepackage[]{xcolor}
% [2017.01.16] Work around option clash:
\definecolor{MidnightBlue}{rgb}{0.1, 0.1, 0.44}

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkred}{rgb}{0.5,0,0}


% Define the language styles we will use
%
\lstset{%
    frame=none,
    rulecolor={\color[gray]{0.7}},
    numbers=none,
%    basicstyle=\footnotesize\ttfamily,
%    basicstyle=\scriptsize\ttfamily,
    basicstyle=\small\ttfamily,
    numberstyle=\color{Gray}\tiny\it,
    commentstyle=\color{MidnightBlue}\it,
    stringstyle=\color{Maroon},
    keywordstyle=[1],
    keywordstyle=[2]\color{ForestGreen},
    keywordstyle=[3]\color{Bittersweet},
    keywordstyle=[4]\color{RoyalPurple},
    captionpos=b,
    aboveskip=1\medskipamount,
    xleftmargin=0.5\parindent,
    xrightmargin=0.5\parindent,
    flexiblecolumns=false,
%   basewidth={0.5em,0.45em},           % default {0.6,0.45}
%    escapechar={\%},
    escapechar={\@},
%    mathescape=true,
    texcl=true,                          % tex comment lines
    showstringspaces=false
}

\lstloadlanguages{Haskell}
\lstdefinestyle{haskell}{%
    language=Haskell,
    upquote=true,
    deletekeywords={case,class,data,default,deriving,do,in,instance,let,of,type,where,IO,ST,STM},
    morekeywords={[2]class,data,default,deriving,family,instance,type,where},
    morekeywords={[3]in,let,case,of,do},
    morekeywords={[4]IORef,IO,ST,STM,STRef,TVar},
    literate=
        {\\}{{$\lambda$}}1
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{>->}3
        {>>=}{>>=}3
        {->}{{$\rightarrow$}}2
        {>=}{{$\geq$}}2
        {<-}{{$\leftarrow$}}2
        {<=}{{$\leq$}}2
        {=>}{{$\Rightarrow$}}2
        {|}{{$\mid$}}1
        {forall}{{$\forall$}}1
        {exists}{{$\exists$}}1
        {...}{{$\cdots$}}3
%       {`}{{\`{}}}1
%       {\ .}{{$\circ$}}2
%       {\ .\ }{{$\circ$}}2
%
%    deletekeywords={insert},
%    deletekeywords={map,sort,zipWith,replicate,Num,Char,Bool,Array,Int,Double
%                   ,sqrt,not,filter,IO,Maybe,Either,quot,scanl,scanr,reverse,fst,id},
%    literate=
%        {+}{{$+$}}1
%        {/}{{$/$}}1
%        {*}{{$*$}}1
%        % {=}{{$=$}}1
%        {>}{{$>$}}1 {<}{{$<$}}1
%        {\\}{{$\lambda$}}1
%        {\\\\}{{\char`\\\char`\\}}1
%        {->}{{$\rightarrow\;$}}2
%        {>=}{{$\geq$}}2
%        {<-}{{$\leftarrow\;$}}2
%        {<=}{{$\leq$}}2
%        {=>}{{$\Rightarrow\;$}}2
%        {\ .}{{$\circ$}}2
%        {\ .\ }{{$\circ$}}2
%        {>>}{{>>}}2
%        {>>=}{{>>=}}2
%        {=<<}{{=<<}}2
%        {|}{{$\mid$}}1
%        {dotdotdot}{{$\ldots$}}3
}

\lstdefinestyle{inline}{%
    style=haskell,
%    basicstyle=\footnotesize\ttfamily,
%    basicstyle=\scriptsize\ttfamily,
    basicstyle=\small\ttfamily,
    %% keywordstyle=[1],
    %% keywordstyle=[2],
    %% keywordstyle=[3],
    %% keywordstyle=[4],
    escapechar={\@},
    mathescape=true,
    literate=
        {\\}{{$\lambda$}}1
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{>->}3
        {>>=}{>>=}3
        {->}{{$\rightarrow$\space}}3    % include forced space
        {>=}{{$\geq$}}2
        {<-}{{$\leftarrow$}}2
        {<=}{{$\leq$}}2
        {=>}{{$\Rightarrow$}}2
        {|}{{$\mid$}}1
%        {~}{{$\sim$}}1
        {forall}{{$\forall$}}1
        {exists}{{$\exists$}}1
        {...}{{$\cdots$}}3
}

\lstnewenvironment{code}
    {\lstset{style=haskell}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    {}

% Default all listings to Haskell style
\lstset{style=haskell}

% \newcommand{\inl}[1]{\lstinline[style=inline];#1;}
\newcommand{\il}[1]{\lstinline[style=inline,mathescape=true];#1;}

\newcommand{\makeatcode}{\lstMakeShortInline[style=inline]@}
\newcommand{\makeatchar}{\lstDeleteShortInline@}


==> introduction.tex <==
%% \NV{Refinement Reflection should be toned down as readers most probably are not familiar with it}
%% \NV{The idea can be explained in 1st intro par without refinement reflection: we could have used a different prover}
%% \NV{Now the story is refinement reflection is implemented, we can to use it to construct proofs}
%% \NV{Proof are tedious we use generics to automate}
%% \NV{How about We have this generic proof generation technique and implemented it using refinement reflection}


\section{Introduction}

Refinement reflection is a technique for extending existing
programming languages into theorem provers~\cite{refinement-reflection}.
\LH~\cite{refinement-types-for-haskell}
implements refinement reflection, thereby allowing
Haskell programmers to verify properties of their
code by writing programs directly in the language.
%
Using \LH's library of proof combinators, one can
construct proofs by using familiar techniques such
as pattern matching and recursion, allowing us to
write proofs as \textit{Haskell} programs (as opposed
to those in a separate proof language).

\LH's refinement reflection is well-suited for verifying
type class laws. Many of Haskell's type classes, such as
@Functor@ and @Monoid@, come with expectations that
instances of those classes will obey certain properties.
%
In standard Haskell, there is no way to be sure that instances actually satisfy
these laws, but with \LH and refinement reflection, it becomes possible.

In practice, deploying refinement reflection can be tedious.
%
Implementing many proofs can involve excessive amounts of
boilerplate code. Even worse, the size of some proofs can
grow quadratically.
%
For instance, if one wishes to prove that an @Eq@
instance for some data type is really an equivalence
relation, proving that equality is symmetric or
transitive can grow extremely quickly due to the
sheer number of cases one has to exhaust.

In this paper, we set out to minimize this boilerplate
and develop a style of refinement-reflection programming
that scales well as the size of a data type grows.
%
To do so, we adapt a style of datatype-generic programming in the tradition of
the Glasgow Haskell Compiler's @GHC.Generics@ module.
~\footnote{\url{http://hackage.haskell.org/package/base-4.9.1.0/docs/GHC-Generics.html}}.
That is to say, for some data type about which we want to prove a property, we
first consider a \textit{representation type} which is isomorphic to the
original data type.
%
This representation type is the composition of several
very small data types. By proving the property in question
for these small, representational data types, we can compose
these proofs and use them to prove the property for the original
data type by taking advantage of the isomorphism between the
original and representation types.

We contribute an application of refinement reflection
to achieve proof reuse and concision, and show how
refining an isomorphism between two data types can
help prove \emph{other} refined properties, such as
verified equivalence relations or verified total
orderings.
%
We provide an implementation of these ideas using
\LH and the Glasgow Haskell Compiler, located at \codeurl.

The contributions of this paper are:

\begin{itemize}

\item We extend Haskell type classes to verified type classes which have explicit
  proofs of type class laws (\S~\ref{sec:motivation}),

\item We propose an extension to GHC generics which adds proofs of isomorphism
  between the original datatype and its representation type, with some machinery
  to automatically derive the proofs (\S~\ref{sec:isos}), and

\item We use the ``generic isomorphism'' machinery to derive verified instances
  for a sample set of verified type classes (\S~\ref{sec:eval}).
\end{itemize}


==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
We begin our discussion of verified type class instances by reviewing some
common classes in the Haskell ecosystem that have proof obligations associated
with them. For instance, a mainstay of Haskell programming is the \texttt{Eq}
class, which represents types which can be checked for boolean equality:

\begin{code}
class Eq a where
  (==) :: a -> a -> Bool
\end{code}

Another common example the \texttt{Ord} class, which provides an
abstraction for totally ordered data types:

\begin{code}
class Eq a => Ord a where
  (<=) :: a -> a -> Bool
\end{code}

We will focus on \texttt{Ord} in great detail this section, as it provides
a convenient case study for verifying type class laws with refinement reflection.
To be a total order, any instance of \texttt{Ord} should satisfy these laws:

\begin{itemize}
\item \emph{Reflexivity}:
  For all $x$, $x \leq x$.
\item \emph{Antisymmetry}:
  For all $x$, $y$, if $x \leq y$ and $y \leq x$, then $x = y$.
\item \emph{Transitivity}:
  For all $x$, $y$, $z$, if $x \leq y$ and $y \leq z$, then $x \leq z$.
\item \emph{Totality}:
  For all $x$, $y$, $x \leq y$ or $y \leq x$.
\end{itemize}

These laws can be encoded via refinement types in Liquid Haskell. We extend the
\texttt{Ord} class to a \texttt{VerifiedOrd} subclass with four more fields:

\begin{code}
class Ord a => VerifiedOrd a where
  refl    :: x:a -> { x <= x }
  antisym :: x:a -> y:a
          -> { x <= y && y <= x => x == y }
  trans   :: x:a -> y:a -> z:a
          -> { x <= y && y <= z => x <= z }
  total   :: x:a -> y:a
          -> { x <= y || y <= x }
\end{code}

Note that the code above is not standard Haskell syntax. Rather, this is the
\textit{refined} version of the class which Liquid Haskell reasons about in
refinement logic. In reality, the code above would be written in a special form
of comment that Liquid Haskell recognizes, and the actual definition of
\texttt{VerifiedOrd} (written alongside the comment) would be written alongside
the comment.

\begin{code}
class Ord a => VerifiedOrd a where
  refl    :: a -> Proof
  antisym :: a -> a -> Proof
  trans   :: a -> a -> a -> Proof
  total   :: a -> a -> Proof
\end{code}

Here, \texttt{Proof} is simply a type alias for the unit type \texttt{()} in
Liquid Haskell's library of proof combinators. Since the proofs carry no useful
information at runtime, the unit type suffices as a runtime witness to a
proof. In the rest of the paper, we will simply refer to the refined definitions
of Haskell classes and functions for brevity.

\subsection{A simple example}
\label{sec:simple-example}

To demonstrate the sort of theorem proving that refinement reflection entails,
we will prove the \texttt{Ord} laws for an extremely simple data type:

\begin{code}
data SimpleA = SimpleA Int deriving (Eq)
instance Ord SimpleA where
  (SimpleA s1) <= (SimpleA s2) = (s1 <= s2)
\end{code}

The reflexivity of \texttt{SimpleA} can be represented with proof combinators
like so:

\begin{code}
simpleARefl :: x:SimpleA -> { x <= x }
simpleARefl x@(SimpleA s)
  =  x <= x
  =. (s <= s)
  =. True
  ** QED
\end{code}

Here, the type signature is Liquid Haskell syntax, and in actual Haskell code
would be placed inside a comment. The implementation of \texttt{simpleARefl} uses
these proof combinators:

\begin{code}
(=.) :: x:a -> y:{ a | x = y } -> { v:a | v = x }
x =. _ = x

data QED = QED

(**): :: a -> QED -> Proof
_ ** _ = ()
\end{code}

The type of the \texttt{(=.)} function checks that the left- and right-hand
sides are equal (according to \texttt{(=)}, the SMT solver's notion of
equality). \texttt{QED} and \texttt{(**)} provide a way to promote a chain of
equations into a \texttt{Proof}. Using these combinators gives refinement proofs
a distinct equational reasoning flavor.

We can prove antisymmetry, transitivity and totality for \texttt{SimpleA} in much
the same way as we did for reflexivity:

\begin{code}
simpleAAntisym :: x:SimpleA -> y:SimpleA
               -> { x <= y && y <= x => x == y }
simpleAAntisym x@(SimpleA s1) y@(SimpleA s2)
  =  (x <= y && y <= x)
  =. (s1 <= s2 && s2 <= s1)
  =. (s1 == s2)
  =. (x == y)
  ** QED

simpleATrans :: x:SimpleA -> y:SimpleA -> z:SimpleA
             -> { x <= y && y <= z => x <= z }
simpleATrans x@(SimpleA s1) y@(SimpleA s2)
             z@(SimpleA s3)
  =  (x <= y && y <= z)
  =. (s1 <= s2 && s2 <= s3)
  =. (s1 <= s3)
  =. (x <= z)
  ** QED

simpleATotal :: x:SimpleA -> y:SimpleA -> z:SimpleA
             -> { x <= y || y <= x }
simpleATotal x@(SimpleA s1) y@(SimpleA s2)
  =  (x <= y || y <= x)
  =. (s1 <= s2 || s2 <= s1)
  ** QED
\end{code}

Since the SMT solver knows how to reason about \texttt{Int}s directly, it can
prove these theorems with relative ease, as evidenced by the fact that we did
not need any lemmas about \texttt{Int} arithmetic.

However, if one makes the definition of \texttt{SimpleA} even slightly more
complex, it becomes apparent that this very direct style of proof does not scale
well. Let's create a slightly modified version of \texttt{SimpleA} with two
constructors:

\begin{code}
data SimpleB = SimpleB1 Int | SimpleB2 Int
  deriving Eq
instance Ord SimpleB where
  (SimpleB1 s1) <= (SimpleB1 s2) = (s1 <= s2)
  (SimpleB2 s1) <= (SimpleB2 s2) = (s1 <= s2)
  (SimpleB1 {}) <= (SimpleB2 {}) = True
  (SimpleB2 {}) <= (SimpleB1 {}) = False
\end{code}

The proof of reflexivity does not change significantly, as it amounts to adding
another case for the additional constructor:

\begin{code}
simpleBRefl x@(SimpleB1 s)
  =  (x <= x)
  =. (s <= s)
  =. True
  ** QED
simpleBRefl x@(SimpleB2 s)
  =  (x <= x)
  =. (s <= s)
  =. True
  ** QED
\end{code}

The proof of antisymmetry, however, becomes a bit more complicated. We now
require a case for every pairwise combination of constructors:

\rgs{Why does LH require that we match on every combination? Why can't we
just use a catch-all pattern here?}

\begin{code}
simpleBAntisym x@(SimpleB1 s1) y@(SimpleB1 s2)
  =  (x <= y && y <= x)
  =. (s1 <= s2 && s2 <= s1)
  =. (s2 == s1)
  =. (x == y)
  ** QED
simpleBAntisym x@(SimpleB1 s1) y@(SimpleB1 s2)
  =  (x <= y && y <= x)
  =. (s2 <= s1 && s1 <= s2)
  =. (s2 == s1)
  =. (y == x)
  ** QED
simpleBAntisym x@(SimpleB1 {}) y@(SimpleB1 {})
  =  (x <= y && y <= x)
  =. (True && False)
  =. False
  ** QED
simpleBAntisym x@(SimpleB1 {}) y@(SimpleB1 {})
  =  (x <= y && y <= x)
  =. (False && True)
  =. False
  ** QED
\end{code}

One thing to notice is that with the addition of multiple constructors, there are
now cases where the hypothesis does not hold---namely, when comparing a
\texttt{SimpleB1} value with a \texttt{SimpleB2} value. Since the hypothesis
reduces to \texttt{False}, the entire implication is vacuously true, so
concluding with \texttt{False} is sufficient for Liquid Haskell's needs.

However, something worrying has happened here. The proof of antisymmetry for
\texttt{SimpleA} only took two cases, whereas the corresponding proof for
\texttt{SimpleB} took four cases. If we were to add a third constructor, then
the antisymmetry proof would take eight cases. In other words, the size
this proof is growing quadratically with the number of
constructors!

The other proofs needed for \texttt{VerifiedOrd} are also quick to grow.
Like antisymmetry, the proof of totality grows quadratically, since it must
consider every pairwise combination of two constructors.
The proof of transitivity has an even more noticeable
increase in code growth, since it must match on the every combination of
\textit{three} \texttt{Simple} values, so while the one-constructor variant of
the proof of transitivity has one case, the two-constructor variant would have
eight cases, and a three-constructor variant would have 27 cases.

Perhaps even more troublesome than the size of these proofs themselves is the
fact that most of these cases are sheer boilerplate. For instance, the proof of
antisymmetry follows a predictable pattern. For the cases where the constructors
are both the same, we compare the fields of the constructors, appeal to
properties of \texttt{Int} arithmetic, and conclude that the two values
are equal. For the cases where different constructors are matched upon,
one comparison will end up being \texttt{False}, causing the whole
hypothesis to be \texttt{False}. This is routine code that is begging to be
automated with some kind of proof reuse technique.

\section{Decomposing the problem, generically}
\label{sec:isos}

Having seen the kind of tedium that writing proofs can entail, we present
a solution. Notably, our approach does not require adding new features to
Liquid Haskell itself---instead, we use techniques that only require some
extensions found in the Glasgow Haskell Compiler (GHC).

We adapt an approach from the datatype-generic programming literature where we
take an algebraic data type and construct a \textit{representation type}
which is isomorphic to it. The representation type itself is a composition of
small data types which represent primitive notions such as single
constructors, products, sums, and fields. We also establish a data type for
witnessing the isomorphism between a data type and its representation type.

With these tools, we can shift the burden of proof from the original data type
(which may be arbitrarily complex) to the handful of simple data types which
make up representation types. Moreover, since \textit{all} data types can be
expressed in terms of these representational building blocks, proving a property
for these data types is enough to prove the property for any other algebraic
data type.

\subsection{A primer on datatype-generic programming}
\label{sec:basic-representational-types}

To build up representation types, we use a generic programming library very
similar to the one found in the standard \texttt{GHC.Generics}
module~\cite{generic-deriving}. First, we utilize a type class which captures
the notion of conversion to and from a representation type:

\begin{code}
class Generic a where
  type Rep a :: * -> *
  from :: a -> Rep a x
  to :: Rep a x -> a
\end{code}

The \texttt{Rep} type itself will always be some combination of the following
data types:

\begin{code}
data U1 p = U1 -- Nullary constructors
newtype Rec0 c p = Rec0 c -- Fields
data (f :*: g) p = (f p) :*: (g p) -- Products
data (f :+: g) p = L1 (f p) | R1 (g p) -- Sums
\end{code}

The roles of these types are best motivated by example. For example, for this
linked-list data type:

\begin{code}
data List a = Nil | Cons a (List a)
\end{code}

We define its canonical \texttt{Generic} instance like so:
\footnote{The actual implementation features another data type, \texttt{M1}, which
is used only for metadata. For the sake of simplicity, we have left it out
of the discussion in this paper.}

\begin{code}
instance Generic (List a) where
  type Rep (List a) =
    U1 :+: (Rec0 a :*: Rec0 (List a))
  from Nil = L1 U1
  from (Cons x xs) = R1 (Rec0 x :*: Rec0 xs)
  to (L1 U1) = Nil
  to (R1 (Rec0 x :*: Rec0 xs)) = Cons x xs
\end{code}

This highlights the purpose of each of the representational building block types.
\texttt{(:+:)} encodes a choice between two constructors (\texttt{Nil} and
\texttt{Cons}). In the left constructor, \texttt{U1} indicates that there are
no fields. In the right constructor, we encounter \texttt{(:*:)}, which denotes
a choice between two fields of the constructor. The first field is
\texttt{Rec0 a}, to indicate a field of type \texttt{a}, and similarly, the second
field is \texttt{Rec0 (List a)}, for a field of type \texttt{List a}.

It should be emphasized that these four simple data types are enough to
represent \textit{any} \HaskellStandard data type. For instance, if one were to add
more constructors to a data type, its corresponding \texttt{Rep} type would change by
adding additional occurrences of \texttt{(:+:)} for each constructor. Therefore,
these four data types conveniently provide a unified way to describe the
structure of any data type, a property which will be useful shortly.

Coming up with \texttt{Generic} instances is itself a source of boilerplate,
but luckily, GHC comes equipped with a \\
\texttt{DeriveGeneric} extension that allows for automatically generating such
instances. However, \texttt{Generic} alone isn't enough for our needs, as we
need to be able to prove that the \texttt{from} and \texttt{to} functions
admit an isomorphism. In pursuit of that goal, we define a subclass of
\texttt{Generic} with two proof methods that express the fact that \texttt{from}
and \texttt{to} are mutual inverses.

\begin{code}
class Generic a => GenericIso a where
  `\tof` :: x:a -> { to (from x) == x }
  `\fot` :: x:Rep a x -> { from (to x) == x }
\end{code}

As one might expect, all \texttt{Generic} instances that \\
\texttt{DeriveGeneric} produces also admit instances of \texttt{GenericIso}.
As an example, we can write an instance for the \texttt{List} type like so:

\begin{code}
instance GenericIso (List a) where
  `\tof` x@Nil
    =  to (from x) =. to (L1 U1)
    =. x ** QED
  `\tof` x@(Cons y ys)
    =  to (from x)
    =. to (R1 (Rec0 y :*: Rec0 ys))
    =. x ** QED
  `\fot` x@(L1 U1)
    =  from (to x) =. from Nil
    =. x ** QED
  `\fot` x@(R1 (Rec0 y :*: Rec0 ys))
    =  from (to x) =. from (Cons y ys)
    =. x ** QED
\end{code}

Again, \texttt{GenericIso} instances are a source of boilerplate. Thankfully,
it is simple to automate creating these instances. Our full implementation
features Template Haskell ~\cite{template-haskell} functionality which, given
the name of a data type, will automatically derive the corresponding instances
of \texttt{Generic} and \texttt{GenericIso}. As a demonstration, all of the code
involving lists in this section could have been reduced to:

\begin{code}
data List a = Nil | Cons a (List a)
deriveIso ''List
\end{code}

\subsection{Proofs over representation types}
\label{sec:product-example}

Having identified the four basic data types which can be composed in various ways
to form representation types, the next task is to write proofs for these four
types. We will do so by continuing our earlier \texttt{VerifiedOrd} example from
\Cref{sec:motivation}, and in the process show how one can obtain a valid
lexicographic ordering for any algebraic data type by using this technique.

The \texttt{U1} data type has an extremely simple \texttt{Ord} instance:

\begin{code}
instance Ord (U1 p) where
  U1 <= U1 = True
\end{code}

The \texttt{VerifiedOrd} instance is similarly straightforward, so we will elide
the details here.

The \texttt{Ord} instance for the \texttt{Rec0} type will look familiar:

\begin{code}
instance Ord c => Ord (Rec0 c p) where
  (Rec0 r1) <= (Rec0 r2) = (r1 <= r2)
\end{code}

This is essentially the same \texttt{Ord} instance that we used for
\texttt{SimpleA} in \Cref{sec:simple-example}, except abstracted to an arbitrary
field of type \texttt{c}. The \texttt{VerifiedOrd} instance for \texttt{Rec0} also
mirrors that of \texttt{SimpleA}, so we will simply define the instance, and
leave out the full details of the constitutent proofs:

\begin{code}
instance VerifiedOrd c => VerifiedOrd (Rec0 c p)
\end{code}

The \texttt{(:*:)} type, which serves the role of representing two fields in a
constructor, is also the simplest possible product type, with two conjuncts.
We can express a valid lexicographic ordering on such a type by first checking
if the left fields are equal. If so, we compare the right fields. Otherwise,
we simply compare the left fields:

\begin{code}
instance (Ord (f p), Ord (g p)) =>
          Ord ((f :*: g) p) where
  (x1 :*: y1) <= (x2 :*: y2) =
    if x1 == x2 then y1 <= y2 else x1 <= x2
\end{code}

It can be shown that given suitable \texttt{VerifiedOrd} proofs for the fields'
types \texttt{f p} and \texttt{g p}, this ordering for \texttt{(:*:)} is
reflexive:

\begin{code}
leqProdRefl
  :: (VerifiedOrd (f p), VerifiedOrd (g p))
  => t:((f :*: g) p) -> { t <= t }
leqProdRefl t@(x :*: y) =
     (t <= t)
  =. (if x == x then y <= y else x <= x)
  =. y <= y
  =. True ? refl y
  ** QED
\end{code}

Note that we use an additional
proof combinator \texttt{($\therefore$)} here:

\begin{code}
($\therefore$) :: (Proof -> a) -> Proof -> a
f $\therefore$ y = f y
\end{code}

One should read \texttt{($\therefore$)} as being ``prove the equational step on the
left-hand side by using the lemma on the right-hand side''. In the case of
\texttt{leqProdRefl}, we were able to prove that \texttt{y $\leq$ y} is
true precisely because of the assumption that \texttt{y} was reflexive.

The proofs of antisymmetry, transitivity, and totality for \texttt{(:*:)} are
quite long, so we have included them in \Cref{product-type-proofs}. Putting
all of these proofs together gives us a hard-earned \texttt{VerifiedOrd}
instance:

\begin{code}
instance (VerifiedOrd (f p), VerifiedOrd (g p))
       => VerifiedOrd ((f :*: g) p) where
  refl    = leqProdRefl
  antisym = leqProdAntisym
  trans   = leqProdTrans
  total   = leqProdTotal
\end{code}

In a similar vein, we can come up with a \texttt{VerifiedOrd} instance for
\texttt{(:+:)}. \texttt{(:+:)} not only represents choice between two constructors,
it is also the simplest possible sum type, with two disjuncts.
A lexicographic ordering on sums is defined so that everything on the left
is less than everything on the right:

\begin{code}
instance (Ord (f p), Ord (g p)) =>
          Ord ((f :+: g) p) where
  (L1 x) <= (L1 y) = x <= y
  (L1 x) <= (R1 y) = True
  (R1 x) <= (L1 y) = False
  (R1 x) <= (R1 y) = x <= y
\end{code}

Here is an example of a \texttt{VerifiedOrd}-related proof for \texttt{(:+:)}:

\begin{code}
leqSumRefl
  :: (VerifiedOrd (f p), VerifiedOrd (g p))
  => u:((f :+: g) p) -> { u <= u }
leqSumRefl s@(L1 x) =  (s <= s)
                    =. x <= x
                    =. True ? refl x
                    ** QED
leqSumRefl s@(R1 y) =  (s <= s)
                    =. y <= y
                    =. True ? refl y
                    ** QED
\end{code}

This might remind you of the corresponding reflexivity proof for \texttt{SimpleB}
in \Cref{sec:simple-example}. This resemblance is intended, as the structure of the
\texttt{SimpleB} data type is quite similar to that of \texttt{(:+:)}. The
remaining proofs for \texttt{(:+:)}, which are also rather lengthy,
can be found in \Cref{sum-type-proofs}). Finally, we obtain the following
\texttt{VerifiedOrd} instance for \texttt{(:+:)}:

\begin{code}
instance (VerifiedOrd (f p), VerifiedOrd (g p))
       => VerifiedOrd ((f :+: g) p) where
  refl    = leqSumRefl
  antisym = leqSumAntisym
  trans   = leqSumTrans
  total   = leqSumTotal
\end{code}

We wish to place particular emphasis on the fact that these \texttt{VerifiedOrd}
instances are compositional. That is, we can put together whatever combination
of \texttt{(:+:)}, \texttt{(:*:)}, \texttt{U1}, and \texttt{Rec0} we wish, and
we will ultimately end up with something which has a valid \texttt{VerifiedOrd}
instance. This is crucial, as it ensure that this technique scales
up to large examples.

\subsection{Reusing proofs}
\label{sec:iso-example}

Given a \texttt{VerifiedOrd} instance for a representation type, how can we relate
it back to the original data type to which it is isomorphic? The answer lies in
the \texttt{GenericIso} class from before. \texttt{GenericIso} has enough
power to take a \texttt{VerifiedOrd} proof for one type and reuse it for
another type.

To begin, we will need a way to compare two values of a type that is an instance
of \texttt{Generic}, given that its representation type \texttt{Rep} is
an instance of \texttt{Ord}:

\begin{code}
leqIso :: (Ord (Rep a x), Generic a)
       => (a -> a -> Bool)
leqIso x y = (from x) <= (from y)
\end{code}

We can straightforwardly prove that \texttt{leqIso} is a total order:

\begin{code}
leqIsoRefl
  :: (VerifiedOrd (Rep a x), GenericIso a)
  => x:a -> { leqIso x x }
leqIsoRefl x =  leqIso x x
             =. (from x) <= (from x)
             =. True ? refl (from x)
             ** QED

leqIsoAntisym
  :: (VerifiedOrd (Rep a x), GenericIso a)
  => x:a -> y:a
  -> { leqIso x y && leqIso y x => x == y }
leqIsoAntisym x y =
     (leqIso x y && leqIso y x)
  =. ((from x) <= (from y) && (from y) <= (from x))
  =. (from x) == (from y)
      ? antisym (from x) (from y)
  =. x == y ? fromInj x y
  ** QED

leqIsoTrans
  :: (VerifiedOrd (Rep a x), GenericIso a)
  => x:a -> y:a -> z:a
  -> { leqIso x y && leqIso y z => leqIso x z }
leqIsoTrans x y z =
     (leqIso x y && leqIso y z)
  =. ((from x) <= (from y) && (from y) <= (from z))
  =. (from x) <= (from z)
      ? trans (from x) (from y) (from z)
  =. leqIso x z
  ** QED

leqIsoTotal
  :: (VerifiedOrd (Rep a x), GenericIso a)
  => x:a -> y:a
  -> { leqIso x y || leqIso y x }
leqIsoTotal x y =
     (leqIso x y || leqIso y x)
  =. ((from x) <= (from y) || (from y) <= (from x))
  =. True ? total (from x) (from y)
\end{code}

Now we put it all together and write the \texttt{VerifiedOrd} instance that
was begging to be discovered:

\begin{code}
instance (VerifiedOrd (Rep a x), GenericIso a)
       => VerifiedOrd a where
  (<=)    = leqIso
  refl    = leqIsoRefl
  antisym = leqIsoAntisym
  trans   = leqIsoTrans
  total   = leqIsoTotal
\end{code}

\subsection{Some complete examples}

With the above combinators, writing a \texttt{VerifiedOrd} instance for an
algebraic datatype amounts to finding an isomorphic representation of the
datatype and using the right combinators to build up the proof from the ground
types. We illustrate this with the following example:

\begin{code}
data Foo = Bar Int Double | Baz Char
  deriving (Eq, Ord)
deriveIso ''Foo
\end{code}

Recall that \texttt{deriveIso ''Foo} generates the following \texttt{Generic}
instance:

\begin{code}
instance Generic Foo where
  type Rep Foo = (Rec0 Int :*: Rec0 Double) :+: Rec0 Char
  ...
\end{code}

This means we only need to write \texttt{VerifiedOrd} instances for
\texttt{Int}, \texttt{Double} and \texttt{Char}, and by type class instance
resolution, we get a \texttt{VerifiedOrd} instance for \texttt{Foo}!

\begin{code}
instance VerifiedOrd Foo
\end{code}

This technique works for recursive datatypes too:

\begin{code}
data Nat = Zero | Suc Nat
  deriving (Eq, Ord)
deriveIso ''Nat
instance VerifiedOrd Nat
\end{code}


\subsection{Aside: universal algebra and model theory}

The idea of proof reuse is motivated from model theory in mathematical
logic. First-order model theory studies properties of models of first-order
theories using tools from universal algebra. In particular, preservation
theorems study the closure properties of classes of models across algebraic
operations. By interpreting Haskell type classes and verified type classes as
algebraic objects, we can borrow these ideas to do generic proving and verified
programming.

A Haskell type class can be interpreted as a signature in the sense of universal
algebra, that is, a collection of function and relation symbols with fixed
arities. Relations are identified with propositions, that is, functions whose
codomain is \texttt{Bool}. For example, the type class \texttt{Eq} corresponds
to the signature $\sigma_{Eq}:=(=)$, and the \texttt{Ord} class corresponds to
the signature $\sigma_{Ord}:=(\leq,=)$. ``Type class laws'', expressed as
first-order axioms using refinement reflection are identified as a first-order
theory, that is, a set of first-order statements (identified upto logical
equivalence). For example, for \texttt{VerifiedOrd}, we have the theory of total
orders given by $T_{Ord}$ with the axioms for reflexivity, antisymmetry,
transitivity, and totality.

We can now interpret building an instance of a verified type class
model-theoretically. A type is an instance of a verified type class, if it forms
a structure in that signature, and is also a model of the first-order
theory. For example, a type $a$ is an instance of \texttt{VerifiedOrd}, if there
are operations $=^a$, $\leq^a$ so that $A:=(a,=^a,\leq^a)$ is a $\sigma_{Ord}$
structure, and $A \vDash T_{Ord}$, that is, $A$ is a model of $T_{Ord}$.

Given a first-order theory $T$ and $K$, the class of models of $T$, one can ask
if $K$ is closed under algebraic operations like products ($P(K)$), coproducts
($C(K)$), substructures ($S(K)$), homomorphic images ($H(K)$), isomorphic images
($I(K)$). The answers to some of these are well known in logic.

\begin{itemize}
\item $I(K) = K$ for any $T$.
\item (\emph{\L{}o\'{s}-Tarski}) $S(K) = K$ iff $T$ is universal.
\item $SP(K) = K$ iff $T$ is a Horn-clause theory.
\item (\emph{Birkhoff}) $HSP(K) = K$ iff $T$ is equational.
\end{itemize}

This gives a firm theoretical foundation for our technique for shorter refinement
reflection proofs. The fact that algebraic operations are closed under
products means that if we can prove a property for two types, then we can
immediately conclude that the property holds for a constructor with those two
types as fields. Similarly, closure under coproducts lets us conclude that if a
property holds for two constructors, then that property holds for a sum type
composed of those two constructors. Lastly, closure under isomorphism lets us
say that if we can prove a property for one data type, then we can conclude the
property for any other data type with an isomorphic structure.

% \subsection{A recursive datatype example}
%
% There is an interesting point to make about recursive Haskell
% datatypes. Strictly positive datatypes in Haskell are interpreted as initial
% algebras, and by \emph{Lambek's theorem}, come equipped with an isomorphism. For
% example, the peano \texttt{Nat} datatype has the following factorization
% $\texttt{Nat} \simeq \mathbf{1} \coprod \texttt{Nat}$.
%
% \begin{code}
% data Nat = Zero | Suc Nat deriving (Eq)
%
% fromNat :: Nat -> U1 :+: Rec0 Nat
% fromNat Zero    = L1 U1
% fromNat (Suc n) = R1 (Rec0 n)
%
% toNat :: U1 :+: Rec0 Nat -> Nat
% toNat (L1 U1)       = Zero
% toNat (R1 (Rec0 n)) = Suc n
%
% `\tof`Nat :: n:Nat -> { toNat (fromNat n) == n }
% `\tof`Nat Zero
%   = toNat (fromNat Zero) ** QED
% `\tof`Nat (Suc n)
%   = toNat (fromNat (Suc n)) ** QED
%
% `\fot`Nat :: n:(U1 :+: Rec0 Nat)
%        -> { fromNat (toNat n) == n }
% `\fot`Nat (L1 U1)
%   = fromNat (toNat (L1 U1)) ** QED
% `\fot`Nat (R1 (Rec0 n))
%   = fromNat (toNat (R1 (Rec0 n))) ** QED
%
% instance Iso (U1 :+: Rec0 Nat) Nat where
%   to   = toNat
%   from = fromNat
%   `\tof`  = `\tof`Nat
%   `\fot`  = `\fot`Nat
% \end{code}
%
% There is a trivial total ordering on the singleton type \texttt{U1}, and it is
% preserved along coproducts, which means we now have a free total ordering on
% \texttt{Nat} too!
%
% \begin{code}
% Zero <= Suc Zero <= Suc (Suc Zero) <= $\ldots$
% \end{code}

